Simulation-Based Performance Evaluation of 3D Object Detection Methods with Deep Learning for a LiDAR Point Cloud Dataset in a SOTIF-related Use Case

Safety of the Intended Functionality (SOTIF) addresses sensor performance limitations and deep learning-based object detection insufficiencies to ensure the intended functionality of Automated Driving Systems (ADS). This paper presents a methodology examining the adaptability and performance evaluation of the 3D object detection methods on a LiDAR point cloud dataset generated by simulating a SOTIF-related Use Case. The major contributions of this paper include defining and modelling a SOTIF-related Use Case with 21 diverse weather conditions and generating a LiDAR point cloud dataset suitable for application of 3D object detection methods. The dataset consists of 547 frames, encompassing clear, cloudy, rainy weather conditions, corresponding to different times of the day, including noon, sunset, and night. Employing MMDetection3D and OpenPCDET toolkits, the performance of State-of-the-Art (SOTA) 3D object detection methods is evaluated and compared by testing the pre-trained Deep Learning (DL) models on the generated dataset using Average Precision (AP) and Recall metrics.

==> Chapters/Chap_acyronms.tex <==
\begin{appendices}
\begin{subappendices}


\section{\uppercase{Appendix}}
%	\addcontentsline{toc}{section}{Appendices}
	\renewcommand{\thesubsection}{\Alph{subsection}.1}
	
\subsection{Abbreviations}
\label{chap_abbreviations}
\begin{acronym}
	\acro{ads}[ADS]{Automated Driving System}
	\acrodefplural{ads}[ADSs]{Automated Driving Systems}
	\acro{ap}[AP]{Average Precision}
	\acro{cnn}[CNN]{Convolutional Neural Network}
	\acrodefplural{cnn}[CNNs]{Convolutional Neural Networks}
	\acro{dl}[DL]{Deep Learning}
	\acro{FN}[FN]{False Negative}
	\acro{FP}[FP]{False Positive}
	\acro{iou}[IoU]{Intersection over Union}
	\acro{lidar}[LiDAR]{Light Detection And Ranging}	
	\acro{mvx-net}[MVX-Net]{Multimodal VoxelNet for 3D Object Detection}
	\acro{part-a2}[Part-A\textsuperscript{2}]{Part-aware and Part-aggregation Network}
	\acro{PointPillars}[PointPillars]{Fast Encoders for Object Detection from Point Clouds}
	\acro{pointrcnn}[PointRCNN]{3D object proposal generation and detection from point}
	\acro{pv-rcnn}[PV-RCNN]{Point-Voxel Feature Set Abstraction for 3D Object Detection}
		\acro{rcnn}[R-CNN]{	Region-based Convolutional Neural Networks }
	\acro{roi}[RoI]{Region of Interest}
	\acro{rpn}[RPN]{Region Proposal Network}
	\acro{second}[SECOND]{Sparsely Embedded Convolutional Detection}
	\acro{sota}[SOTA]{State-of-the-Art}
	\acro{sotif}[SOTIF]{Safety Of The Intended Functionality}
	\acro{tcp}[TCP]{Transmission Control Protocol}
	\acro{TN}[TN]{True Negative}
	\acro{TP}[TP]{True Positive}
	\acro{v2v}[V2V]{Vehicle-to-Vehicle}
\end{acronym}


\end{subappendices}
\end{appendices}

